Monitoring Auditable Claims in the Cloud

When deploying mission-critical systems in the cloud, where deviations may have severe consequences, the assurance of critical decisions becomes essential. Typical cloud systems are operated by third parties and are built on complex software stacks consisting of e.g., Kubernetes, Istio, or Kafka, which due to their size are difficult to be verified. Nevertheless, one needs to make sure that mission-critical choices are made correctly. We propose a flexible runtime monitoring approach that is independent of the implementation of the observed system that allows to monitor safety and data-related properties. Our approach is based on combining distributed Datalog-based programs with tamper-proof storage based on Trillian to verify the premises of safety-critical actions. The approach can be seen as a generalization of the Certificate Transparency project. We apply our approach to an industrial use case that uses a cloud infrastructure for orchestrating unmanned air vehicles.

==> TODO.tex <==
Intro
    - Revisions als Hauptbeitrag drin?
    - Link zu security? Hauptthema der Konferenz

Related Work
    - ok?
    
Evaluation, e.g. after 100 requests
    - What is the monitoring overhead? 
        - CPU: Datalog Interpreter
        - Latencies: beause of forwarding to security monitor, possible to make asynchronous)
        - KB size/RAM
        (- Which improvement using next rules? Storage difference, Number of facts)
        % - Latencies when running in active mode? (actually does not work as seen in Demo?) -> 
    - Delay events kommen mehrfach vor
Discussion
    - Monitor können in authorization mode laufen
    
Next-Rules
    - Next-rules für externe claims?
     - Schwierig zu definieren; wenn Regeln fehlen, 
     fehlt in commits evt. Info von anderen Monitoren
     - Fakten, die nur ein anderer Monitor braucht, müssen mit allen geteilt werden? (FM attests heliport)

Figures
    - Update Fig 2. Interaction agent
    
Sonst
    - Claims werden nicht signiert?
    
Code
    - Link zu Monitor Implementierung bzw. folgendes repo benutzen: https://git.fortiss.org/sorokin/cyberlog-monitoring
    - Nur Regeln/Eine deployment Datei je Service zeigen

Lev
    - Attestations umschreiben
    - Evaluation zu Ende machen
    - update revision picture

Threat model
    - communication channels:
        - modification of events is identified (signature)
    - private key of service disclosed:
        - detectable when correponding rule contains principal whose key is not disclosed
    - compromised monitor that add facts in modified form:
        ??
    - compromised services that add direct facts:
        - not detectable
    - compromised frontend centralized log:
        -> discussion

Final
    - Cyberlogic erwähnen?
    - Ist Datalog mit attestations ein Beitrag, wenn es schon Cyberlogic gibt?

----------- Follow Up Todos ------------

- Required amount of storage is still not constrained
    - calculate how man facts are generated for a request
    - use notion of sessions
        - attacker can create artifical requests/sessions
            - how to cope with?
    - mention explicitly in SB that 
        - not more then X requests will be send
        - external filtering detects incorrect requests/limits number requests
    - Analyse vom notwendigen Speicherbedarf -> Dann Einschränkung über filter
    - Konstante gibt maximal Speicherverbrauch an   
    
- Evaluation
    - fix bug where monitors are not accessable after some requests
       - performance issue?
    - simplify rules for evaluation
    - evaluate required storage for N requests
 

- Improve Language Syntax?
    - specific templates to formulate specific requirements (as EARS)?

- Threat Model

- Story: Concentrate on Runtime Monitoring or on generalization of Certificate Transparency 
    - Checksum DB audit
    - Firmware Transparency
    
------------------------





==> cfp.tex <==
https://conferences.computer.org/cloud/2023/cfp/

Cloud Security
    Confidential Cloud Computing and Trusted Cloud Environments
    Access Control, Authorization, Authentication
    Assurance, Audit, Certification, Compliance
    Fault Tolerance, High Availability, Reliability
    Privacy-aware Data Management
    Cloud Applications of Distributed Ledger Technologies
    
Page limits

Every "Regular Paper" manuscript can include 7 to 10 pages for the main contents (including all text, footnotes, figures, tables and appendices) with additional pages for appropriate references.

Every "Short Paper" manuscript can include 4 to 6 pages for the main contents (including all text, footnotes, figures, tables and appendices) with additional pages for appropriate references. Although the focus is narrow, “Short Paper” submissions must present factual nontrivial research results. Per reviewers’ comments, a “Regular Paper” manuscript may be conditionally accepted as a “Short Paper” should necessary content improvements and length reduction be able to be done in time.

Every “Work-in-Progress” (WIP) manuscript can include up to 3 pages (including main contents and references). WIP manuscripts must present innovative ideas with promising impact. Per reviewers comments, a "Regular Paper" or "Short Paper" manuscript may be conditionally accepted as a "WIP Paper" should necessary content improvements and length reduction be able to be done in time.

--------------
--------------
International Conference on ICT Systems Security and Privacy Protection IFIP SEC 2023, 14-16 June 2023
--------------------
The IFIP SEC conference is the flagship event of the International Federation for Information Processing (IFIP)
Technical Committee 11: Security and Privacy Protection in Information Processing Systems (TC-11).
We seek submissions from academia, industry and government presenting novel research on all theoretical
and practical aspects of security, privacy protection in ICT Systems and cybersecurity of new Internet technologies. We
are especially interested in AI (Artificial Intelligence) and big data analysis supporting security aspects.
Practitioners and industry representatives are encouraged to submit papers
-----------
Paper submission
----------
Submitted papers must be original, unpublished, and not submitted to another conference or journal for
consideration. Accepted papers will be presented at the conference and included in the conference proceedings
published in the IFIP AICT series by Springer Science and Business Media.
All papers must be written in English. Submissions should be at most 14 pages long in total including references
and appendices. Submissions should not be anonymised. PC members are not required to read the appendices, so the
paper should be intelligible without them. Authors must follow the Springer LNCS formatting instructions.
Each paper will receive at least three reviews. At least one author of each accepted paper must register by the
early registration date indicated on the conference website and present the paper. For each accepted paper, at least
one full registration is necessary.

Papers have to be submitted via the Easychair.


==> content/discussion.tex <==
\section{Discussion}

One of the limitations of our approach is to deal with a threat, where all private keys for signing claims get stolen and an attacker creates all required evidence for an event (the attacker knows the contracts). Technical challenges that are not considered in our approach are: (1) The user needs manually to define which events have to be logged, since logging all events is not feasible.
% We have planned to automatically generate Cyberlog programs from the API and Business Logic provided.
(2) Another question is how to determine the order of events when no global clock is used? 
Also, organizational challenges have to be considered: 

(1) Trust is required that a party agrees to launch a monitor and communication is logged correctly and 

(2) information processed by a component could be confidential, and only accessible by authorized components; this can make it impossible to use events as evidence for claims. 

Furthermore, a basic assumption of implementing a claim/evidence database with a centralized storage like Trillian is that the database is operated by a reliable party. 
It is possible to store Trillian logs redundantly to be robust against failures. It is also possible to maintain copies of the log at different parties but manually intervene in case of storage inconsistencies. To identify a compromised claim database that presents a record to different parties differently (split view attack), it is possible to use gossiping as proposed in \cite{gossipTrillian20}. The performance of such solutions needs to be evaluated when it is used in connection with monitoring.
% required to detect a compromised claim database that presents a record to different principals differently
% This can be achieved by gossiping log information as proposed in. This is especially  (split view attack). 
% It is possible to store Trillian logs redundantly to be robust against failures. It is also possible to maintain copies of the log at different parties, but manually intervene in case of storage inconsistencies. This can be achieved by gossiping log information as proposed in \cite{gossipTrillian20}. This is especially required to detect a compromised claim database that presents a record to different principals differently (split view attack). The performance of such solutions needs to be evaluated when using in connection with monitoring.
Also, the revision model and the next rules are not sufficient to avoid that the size of a KB exceeding a threshold. When e.g., a next rule for a service request exists then for every new service request the KB will grow. The reason for this is that old service requests remain in the KB.
% The size of the knowledge base depends mainly on the facts that are directly added to the KB of a monitor, e.g. API requests.
One option to tackle this is to constrain the number of possible bookings for a fixed time interval.% I.e. the assumption would be that a requests is not passed to the RTAPHM system if a maximal number is exceeded. 
% For instance, when we consider the latest allowed UAV start is in two months, and two UAV missions per hour can be launched, then one could allow maximal 2880 service requests to be passed to SB in this interval. 
It might be required additionally to establish a notion of a session so that claims which belong to a completed session can be deleted from the KB.
Considering the expressiveness of the specification language, using Cyberlogic we cannot express negated properties as Datalog does not allow it. However, it is possible to specify rules with negation over claims in a revision, since a revision is immutable. It is future work to extend the language to support this.

\begin{itemize}
% \item private keys get stolen
% \item accessability (rights to launch a monitor)
% \item confidentiality of logged information
% \item centralized log
\end{itemize}
% Another issue is that the claim database poses a SPOF and could presents a record to different
% principals differently.  
% An additionally auditing of the logged data can required The performance is to be evaluated,
% since stored information at each log has to be compared, when, e.g., several centralized logs are deployed in parallel.

\end{itemize}

==> content/introsketch.tex <==

% Story:

% Überwachung notwendig
% Existierender Monitoring Ansatz? 

- Related Work. extra sections
- Marshas Paper: ihr Ansatz ist in unserem Ansatz enthalten
- SIEM Paper? nachträgliche Überprüfung, Komponenten sollten Ergebnisse der Sicherheitsanalyse für Entscheidungen kennen
- Regulatory Compliance. Auditability of actions
- Wir können CT nicht nehmen; verlassen auf "wahre" Daten


% System uses off the shelf components, e.g., as know for systems deployed in clouds.

Clouds systems are a fundamental part of the daily lifes, they are used in terms of inter-organizational web services as \cite{X,Y}, cross-organizational cloud systems \cite{X} in the healthcare, financial or automotive domain /cite Tesla.
eE

The deployment of services in the cloud has to face several risks as hardware, software faults or cyber attacks that can have an impact on the integrity of processed information or the availability of a service. Also in general, such system use open source-software, which is
vulnerable to software supply chain attacks \cite{supply-chain-attacks}, being at the same time not verifiable because of the vast amount of lines
of code. Deplyoment of safety- and security critical systems in the cloud might face therefore sever consequences. Further the auditability of system events is crucial to meet compliance requirements or to have evidence when a systems property is violated and the responsible party or systems component needs to be identified \cite{}.
% Auditability is required also for monitoring to assure that the reasoned verdicts are correct.
% [[State of the Art Cloud System Monitoring/ SIEM]]
\TODO{Check for a better argumentation with SoT}

A default approach to tackle this issue is to monitor the system by aggregating logs from all related system components, correlate data and analyse for anomalies. This is known as Security Information and Event Management (SIEM) \cite{}. 

When an anomaly is detected the monitoring system triggers an alert or automatically reconfigures the system under observations to avoid further harm. Such approach does not give the system components the flexibility to act based on the monitored systems state. Considering the auditability aspect, approaches exist for specific use cases to enable the reasoning based on auditable data, as \cite{certificateTransparency,trillianExamples,Prybila2020RuntimeVF} but are not applicable to a broad range of distributed systems. Another issue is the formalization of the behaviour to be monitored: other existing approaches rely on formalizing the behaviour in form state machines whose application is limited on dynamically monitoring single process instances \cite{rtConversationChechik}. Building a state machine that considers all possible system states is complex. 


==> evaluation/feedback.tex <==
Theo 11.03.23
------
Page 5: “In the rules, we allow the user to write short a for self attests a” But, a could also mean a valid atom in Cyberlogic. Is it intentional that your program is by default Cyberlogic, i.e., everything is attestation. 

Page8: you wrote “Auditability of claims is then enabled in the following way: (1) For claims derived using rules, the evidence is the instance of the rule used to derive the claim.”
I believe, instance of the rule should rather be an argument for the derived claim “justifiable/auditable” – do these two things mean the same? “auditable claim” implies “justifiable claim” 
But, “justifiable claim” may not always imply “auditable claim” Auditability entails structure of the claim-argument-evidence plus a replying mechanism.

------
Vu 11.03.23
-----------------
ok. also Einleitung finde ich, man könnte das Problem mit Cloud etwas spezifischer benennen. An sich ist es ja nicht die Cloud das Problem, sondern ein System, welches in mehrere Komponenten/Services schneiden lässt, kann in die Cloud schneller und unabhängig von einzelne Komponenten deployt werden. Dadurch entstehen komplexe verteilte Systeme. Die Orchestrierung/Koordinierung wird komplexer.  Distributed System hast du auch in deiner Einleitung genannt. Und das finde ich ist das Hauptproblem.

_________________
Radouane
05.03.2023
--------------------------------
The paper is well structured and the problematic and contributions  are well illustrated. 

I have just a few points:

1. In page5, last paragraph, the notion of attestation is not well defined, I think it is better to add some formal description about it.
2. In page6, line 24 of Listing 1.1, I think it should be: DelyTime < 1000
3. In page6, you listed: “The claim good_rtf_exist is generated whenever the facts in the body of the rule are available.” → I think you should rephrase this sentence.
4. In page8, you didn't explain how you use inclusion proof to check that the claim is stored in the DB.5. More experimental results should be added.

Minor rmks:

Page3, in the outline, you listed that section 2 provides an overview of the related works which is not the case.
Page5, last paragraph, “In order to be able to be applied”
Page11, first paragraph, “Should be not removed”
Page11, paragraph Could integration, “whose behaviour the observe”
Page12, paragraph Monitoring Dashbord, “a systems property is violated”

-----------------------------------------
=== Reviewer 1 ===
This paper addresses the objective of auditing huge processed events in distributed systems at runtime, in a generic way.
According to the authors, Runtime auditing of distributed systems is motivated by the need to react immediately in case of misbehavior. One of the requirements of such an auditing process is scalability.

The proposed solution is built on 4 steps. The first one consists to express the monitorable properties in a specification language. The second consists in choosing a verification mechanism. The third is to generate a suitable monitor according to the rules specified in step 1 and finally, the last step consists in storing all the events in a common legger for further verification.

The originality of this solution is in its ability to adapt to different situations but the paper do not give any insights into the requirements a system should have to be a candidate to such a system.

Moreover for step 2: which solution is better for which situation? is it an objective to fix that during the thesis?

The paper is interesting but the scope of application of such a solution should be more precised.


Some points to enhance the paper

- the paper outline is missing: is this necessary?

Score: weak accept

=== Reviewer 2 ===
# Strengths:
- The auditability topic is very interesting
- The paper proposes advancing auditability by moving from a posteriori auditability to online auditability.
- The authors have already implemented a prototype with some components already in place (e.g., Datalog and Trillian).

# Weaknesses:
- The title is too generic for what the paper actually proposes.

- The fault model could be more elaborated. For instance, is it reasonable trusting the cloud to run unreplicated monitors if clouds are untrusted to run unreplicated distributed programs? good point

- It is unclear why other solutions cannot be adapted to audit systems in runtime.

- The system seems to work only on auditing web services, which is a system model restriction that prevents auditability in many other systems that do not use web servers.

- In practical terms, the costs of runtime auditability may be too high. What are the properties that influence this performance? (e.g., the size of the logs? the complexity of log records?)

- What is the required event ordering (e.g., strict, causal)? Can logical clocks solve the problem with the order of events?

- What is the security impact of providing the services' private keys to Kubernetes?

# Typos:

- Some references (e.g., [18, 24]) do not have where they were published.

# Score: weak accept


=== Reviewer 3 ===
The paper presents an interesting idea to make distributed systems auditable at runtime by using distributed monitors.
The idea is interesting and the paper is well written  ( also including some research questions).
On the other hand, the work is really preliminary work. The paper is not supported by quantitative data and it is not clear if some experiments using real-world data are performed to prove the validity of the approach compared with existing solutions.

Strenghts
    -The paper addresses an interesting topic
    -The paper is well written

Score: borderline paper
---------------------------------------------------

==> old/proposal/sota.tex <==


\section{State of the Art}

In this section we want to outline the state of the art in runtime verification, auditability and the related property accountability in DS under the consideration of the aforementioned challenges in the last section.

% To understand given approaches we describe in short the basics of RV:
% The actual process of runtime verification is usually done in a three-step approach \cite{rv_intro}: First a monitor is synthesized from the given property specified e.g. in a logical language. Specification
% languages can be regular, which includes temporal logic (e.g. LTL), regular
% expressions, state machines, but also non-regular, which includes rule systems or stream languages.
% After that, the system to be observed is instrumented to forward events to the monitors. This can happen in an online setting during the systems execution using an asynchronous or synchronous setup, or  an offline setting, where events are stored in a log file to verify rules after the execution. 
% In an offline setting monitors can not trigger enforcement mechanisms if a property is violated, they can just rather pass information that violation took place. Finally in the third step, the actual monitoring process is executed, i.e. the observation of sequences of events (traces) where monitors emit verdicts for a checked property takes place.

% From the architectural point of view online monitoring can be done outline or inline. In the first case that means that the monitor runs in parallel with the application but is not part of the application. Communication to the system has to be done here synchronously or asynchronously, while in the other case the monitor is embedded into the application.

% Originally, synthesis of runtime monitors has been implemented for monolithic systems for avionics technology, consider e.g. the Temporal Rover or Tool Java Path Explorer \cite{synthesis_central} for the synthesis of RV Monitor from LTL Specifications. Both tools were limited on propositional specifications. The last tool could detect race conditions and deadlocks by analyzing single execution in Java programs. 
% Later, parametric specifications were possible, aspect oriented programming has gained interest to instrument systems in a way that decouples the to be monitored code from the monitor. A popular and considered as the fastest centralized RV framework is e.g. MOP. MOP was implemented in JAVA and enabled synchronous and as well asynchronous verification with AspectJ \cite{}. The problem of aspect oriented programming approaches is the overhead through the instrumentation and the bad transparency for debugging of the executed code, since aspect code is specified not directly in the systems implementation but weaved later after compilation. Later also rule based approaches where proposed with tools like LogFire \cite{}, Drools \cite{}  or RuleR \cite{} with a intuitive specification language, considering also internal DSL (monitors are written in same language as the monitored component), but only limited for centralized systems. 

% Later due to the rising demand of distributed systems and evolution of SOA and microservices research in distributed verification became more and more important \cite{}.

% state of the art in runtime verification of web services?

% \subsection*{Centralized Approaches}

% We list here the main related works considering centralized RV approaches:

% Basin et al \cite{basin_monitoring} describe an algorithm for monitoring distributed systems that exhibit partially ordered traces applied for the compliance checking of system executions with data usage policies. Their work is based on the fact, that even if systems have synchronized clocks, distributed components could produce events with the same timestamps. They define a metric temporal logic MFOTL to specify policies and verify those centralized after all locally produced logs are merged. The problem of this approach is the central aggregation of the log for the final verification, since poses as a single point of failure.

% The authors in \cite{cotroneo2020runtime} consider a stream based infrastructure for the collection of event information for a final centralized verification of policies written in EPL from a black-box execution of a cloud-infrastructure system. EPL is a default SQL-like language that is common in CEP Systems. Their approach considers learning policies from fault free traces to detect incorrect systems behaviour. The CEP Engine verifies at the end the EPL rules. While this avoids high coupling of the DS with the monitoring system, this lacks of verification of policies that need to be enforced immediately like in a security critical systems required. They work also do not consider faulty logging and they present their stream based approach on a very limited number of subsystems. Nevertheless the work inspired us to use an event based approach in our proposal.

% In \cite{rtConversationChechik} the authors propose a lightweight runtime monitoring approach for web services to verify liveness and safety properties when only interfaces are known. As specification language they use a subset of UML 2.0 sequence diagrams and convert it to state automata.
% Their specification language eases the use of their tool for non-formal method experts, but their approach is limited on specific properties and is centralized.

% \subsection*{Distributed Monitor Synthesis}

% \subsection*{Decentralized Approaches}
% Several approaches has also tackled decentralized RV.

% \subsection*{Failure-aware Runtime Verification}
 
%  Some works go into direction how to deal with incomplete information due to network failure or component crashes and define more than 2-valued logics. The authors in \cite{Basin2015FailureawareRV} present an approach for the case that whole system components fail or messages are reordered using three valued metrics temporal logics. With the third logical value they model knowledge gaps. 
 
%  The problem of verification with such logics is that statement can only be made whether based on prediction of values or incomplete knowledge with a very course verification result (undefined reasoning: if a system is not sure whether property is fulfilled, it reports "undefined") . Such undefined reasoning do not help to take the right decision to act, unless in a pessimistic way to mine this as negated.
%  Other works \cite{fraigniaud:hal-01011079} consider to get (correct) information through communication with other monitors by replicating observed information in advance, if a specific component fails.
% We do not want to consider failures of entire components, more we want to prevent the components to fail entirely.



% \subsection{Transparency and Auditing in DS}
\subsection{Auditability and Accountability in DS}
We give a short definition of the system properties accountability and auditability in our paper to point out the difference before we provide related work.

\textbf{Accountability} has no uniform definition, it is slightly understood and realized differently, depending on the context or system it is applied for.
 The informal description  "being called account for one's actions" basically gives the idea of the expression. Initially, the term accountability is rooted in ethics and politics from the 17th century, when official representatives had to justify their actions to their rulers \cite{kaciankaAccountability}.  In computer science it is been used in several domains, basically it started for aiming on maintaining privacy on the internet and implementation of e-voting systems.
Since several years it attracted interest in distributed and cloud systems \cite{cloudFramework} when no direct control over the own data is possible or when the SLAs between the client and the cloud provider are not met, and a solid evidence is required when a dispute arises.
The authors in\cite{accountableCloud} defined a cloud system as accountable, if the following is implemented:\textit{ Identities, secure records, auditing and evidence}. Identities enable linking events to parties and secure records enable storage of past events such that tampering is detected. Auditing enables to verify the correctness of secure records, while evidence is related to auditing and means that every claim produces evidence that can be reviewed by third parties independent of the auditor that detects the faulty claim.

\textbf{Auditability} or verifiability is a weaker form of accountability as described in \cite{auditability09}. There it is defined informally  as following: a system is "[... \textit{auditable if, at any audit point, an impartial judge is satisfied with the evidence produced by the [system]}]".
In our setup we consider that a DS is auditable if every participant but also external observer is able to verify whether a (distributed) property of the system is valid or not. We consider to use to use this terminology when we do not regard the blaming of principals explicitly, what characterizes accountability \cite{accountabilityKuesters10}.

% \textbf{Transparency} is linked to auditability can be considered as a requirement for auditability, i.e. to verify the correctness of properties of a system events should be made visible to parties.

A significant approach for implementing an auditable execution of DS has been presented as a first practical work with PeerReview in \cite{peerreview} using tamper-proof storage (later extended by \textit{FullReview}), focusing on the detection of byzantine faults. The algorithm can be described as follows: each component stores in the logging step locally in an append only secure log all messages it has received or send. Entries in the log are signed by each component with a cryptographic hash, so that tampering of entries can be detected. A predefined number of other components can verify the logged events using the hash. To ensure that actually all events are logged, the commitment protocol verifies that a receiver has logged the transmission of a message. Later, in the auditing step, so called \textit{witness} nodes replay the actions in the log on a reference implementation. This makes it possible to locate deviations between the events in the log and the expected output of the reference implementation.

% TO BE CHECKED
The difference of their approach to our requirements is that they do not target verifying distributed properties and they require to have access to the code to instrument the system under observation, while we consider to have a blackbox system with the specification of the service endpoints.

 Another work from the business process management domain \cite{Prybila2020RuntimeVF} has applied blockchain for a distributed verification of business processes. Logs in a blockchain are transparent for all users and the performance is limited a number around 800 transactions per second \cite{}. Their approach cannot enforce policies and is limited to business processes and applications on special domains like logistics or banking and sacrifice with the confidentiality of data. The authors also do not provide an approach how to generate local monitors from a global property specification.

Another popular and successful example implementing and applying auditing is the Certificate Transparency (CT) framework by Google \cite{certificateTransparency}, that was accepted as an experimental standard by IETF. The idea behind CT is to record all issued certificates by publicly trusted certificate authorities (CA) to identify efficiently mistakenly or maliciously issued certificates. The motivation for that initiative was initially the incident when the CA DigiNotar was compromised in 2011 and more than 500 certificates where maliciously issued.
The approach to detect that is the following: all publicly issued certificates need to be logged in a read-only, tamper-proof log.  Domain owners use then monitors to detect incorrect created certificates for their domain, while some auditor nodes monitor the integrity of the log to make manipulation of the log and the stored certificates impossible.
This approach is limited for verifying certificates and cannot be extended that simple for verifying properties of distributed systems as in our use case.Further similiar trillian application has been presented for the detection of malicious of Firmware updates \cite{trillian_ft}, detection of corrupted go packages \cite{sumDBTrillian} provided by module proxies, as well other package mirrors \cite{Hof2017}.

E.g. in \cite{VamsHicks2018} 
 the authors propose a system configurable with Trillian as well as Hyperledger Fabric for achieving transparency in a platform where sensitive data is shared (e.g. healthcare records or communication data), i.e. the system allows individuals to know how their is processed and enables auditors to detect violations of data processing policies. The results show the advantages of using Trillian instead of Distributed Ledger Technology.
 Their paper do not capture methods for the specification of to verifiable properties for monitor generation.

One other inspiring work is the Open Policy Agent (OPA) \cite{opa} framework that, it does not provide any transparency or auditability to the system, but it enables the enforcement of policies across DS. The policies can be specified independent of the component code using the execution of a daemon or proxy containers. OPA is a general purpose policy engine but is mainly focused on the enforcement of authorization policies and deployment policies in cloud native environments. OPA provides also an intuitive and simple way of specifying polices in the declarative datalog like language Rego \cite{rego}. Nevertheless there is the lack of enforcing distributed properties e.g. related to the execution order. 

Our idea is mainly motivated by Evidentia \cite{evidentia}, that has been proposed as a framework for the execution of distributed evidential transactions. Evidentia consists of three different layers: The datalog based cyberlogics language - a logical framework for the definition of policies - the core component Evidential Tool Bus (ETB) \cite{ETB13} and lastly a verifiable distributed ledger. ETB  has been originally implemented as a continuous tool integration framework to generate assurance cases for mission critical software. Here it is used to execute the business logics and generate claims for service executions of distributed components. To enable this, each component incorporates an monitor that executes a service of a given workflow. The workflow needs to be predefined and the execution triggered by querying. The results of the execution are stored in the verifiable ledger. This resulting artifacts /claims that are continuously produced can be reviewed by all stakeholders.
Considering the technical part, Evidentia execute workflows in a top-down manner using Backward Chaining, i.e. after the rule with the head is identified, the algorithm tries to find a solution for the subgoals in the body, if the predicate is a service than the corresponding service is triggered to produce the facts.

Services are therefore considered to be given to execute a workflow.
This approach can not be applied straightforward for the distributed verification of policies, since facts (the services) in the system are dynamically and verification would need to be triggered only if the corresponding facts of a "verification-rule" do exist, i.e. bottom-up. 
The authors also rely on using hyperledger for storing the evidential information, what causes a performance issue similar to the approach \cite{Prybila2020RuntimeVF} when monitoring policies at runtime.

% User-Interfaces for runtime verification

% Some specification languages like BPMN can offer itself a user inuitive specification formalis, but often the domain specific languages are not intuitive enough. Several works are considering in general the synthesis of natural languages to LTL properties \cite{}, but not many tools addressing user interfaces for runtime verification frameworks. 

\subsection{Distributed Monitor Generation}




Existing RV solutions for distributed systems can be classified as $choreography$ or $orchestration$ approaches. In a choreography setup the initial property is broken down and sub parts of the property are verified locally at the components' location, whereas in $orchestration$ approaches one central monitor administrates on a remote location the verification of the property and the collection of events that are required for verification \cite{Francalanza2018}.
We do not consider here approaches for the latter one, since such centralized setup provides no efficiency in terms of message passing and creates a single point of failure.


Presented approaches for the generation of distributed monitors from global properties mainly focus on specifications based on temporal logics.
Especially in the context of LTL there has been also the definition of the so called $migration$ approach, where a formula is passed along the network to collect incrementally all verdicts \cite{localMonitorSynthesis}.

% In the latter case components can be at the same place as the monitors or deployed at a different position. Distributed verification techniques furthermore differ in the aspect of the level of intrusiveness and in the amount of information of the verifiable systems exists, i.e. black-box vs. white-box system. 

As one of the first decentralized RV approaches was proposed by Sen et al. \cite{sen_decentral} for the verification of safety policies using the modal logics pt-DTL (past time distributed temporal logics). With pt-DTL monitors are directly referenced in the specification of a property, what facilitates the monitoring since no central snapshot of the DS is required compared to monitoring LTL specifications. The assumptions for this approach are that communication is asynchronous and components do not share a global clock. The approach is the following: each component has a monitor that has to retrieve information from other monitors when it requires facts that are not part of its responsibility. For this, messages are piggybacked at default business logics messages. Each monitor maintains for all attributes in the system a table of values  and its version (knowledge vector), to maintain synchronisation.
One main problem of this approach is that messages has to be send often to synchronize on the systems states. If no communication takes place, no correct verification is possible. Another problem is that the monitoring code is weaved into the (Java) Byte Code after compilation of the DS program, what creates a coupling between the system under observation and the monitors. 

Borzoo et al. present in \cite{borzoo_decentral} an improvement of the prior approach where events are partially ordered. An implementation and a use case in large distributed systems is not provided.

Another work by Bauer et. al \cite{bauer_decent} is facing the efficient distributed synthesis of monitors from LTL specifications based on execution traces. Their approach use formula progression (rewriting)  to propagate verdicts to the monitors, what can be classified as migration. They validate the efficiency of their framework by comparison to a centralised monitoring approach.
The main problems of their approach is on the one hand the assumption that communication between components is synchronously as common in automotive systems, and on the other hand that events between components are considered to be disjoint. The implementation of their approach was published, but is also not accessible now.

 %His approach requires causal ordering, and cannot express policies on events that are partially ordered, i.e. not related.

One other work \cite{localMonitorSynthesis} that can be considered as an improvement of the prior approach is also considering  generation of local monitors from LTL formulae, but based on a hierarchical monitor setup (choreography). Monitors verify only a designated part of the property formula and propagate their result to their parent monitor. The parent monitor collects the verification result of their children to evaluate their sub part of formula and propagate it to their parent monitor. This approach assumes that the monitors communicate directly without incorporating any secure logging or further requirements for transparency.

The presented and other existing approaches focus on the efficient and sound synthesis of distributed monitors. But for the best of our knowledge no implementation exists, that is used code-independent on a large scale in combination with transparency and auditing.

\subsection{Property Specification}
% Before we have mainly described technical aspects of the monitor generation for a distributed and accountable runtime verification. One needs to consider that the input for the generation needs to be provided by the developer or system provider to enable the accountable monitoring. 

% In the last section we have seen that is common in RV to rely on temporal languages, e.g. LTL as a legacy from the static verification. Properties in such languages are hard to formamlize for people without logical knowledge.
Only a few papers are providing a simplified  formalisation language for distributed properties in monitoring frameworks in the context of runtime verification.
In \cite{rtConversationChechik} the authors therefore present some algorithm to generate monitors (non deterministic finite automata) from UML 2.0 sequence diagrams based on Property Specification Patterns (PSP) \cite{psp} for monitoring global liveness and safety properties of web services. 

 PSP has been proposed for the finite state verification to assist the formulation of model checking properties by providing mappings to several logical formalisms. PSP are characterized  by order patterns which talk about the relative order events can occur, e.g. event A has to occur after C or event B has always to occur before C, and occurrence patterns, which talk about the fact that an event occurs during system execution, e.g. A will never happen or B will always happen. Pattern are associated with scopes, the timeframe they are valid (e.g. before event A or after event B).
 
But the approach in  \cite{rtConversationChechik} do not enable monitoring of several instances of the same process type and performs the monitoring centralized.

==> review_IFIP_SEC.tex <==
Dear Lev Sorokin,

I hope this message finds you well. On behalf of the organizing committee, I would like to express our sincere gratitude to all of you for submitting your work to our conference. We truly appreciate your dedication and effort in contributing to the advancement of knowledge and research in your respective fields.

The review process has been completed. We received a large number of high-quality submissions, and unfortunately, we could not accept them all.

We encourage you to continue your research and consider submitting your work to other conferences or journals.

Once again, thank you for your submissions.

Best regards,

Anna Grocholewska-Czuryło
Chair of the Conference Organizing Committee

SUBMISSION: 5585
TITLE: Monitoring Auditable Claims in the Cloud


----------------------- REVIEW 1 ---------------------
SUBMISSION: 5585
TITLE: Monitoring Auditable Claims in the Cloud
AUTHORS: Lev Sorokin and Ulrich Schöpp

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
The paper proposes a flexible runtime monitoring approach for mission-critical systems running in the cloud that is independent of the implementation of the observation system, using the RTAPHM project as a use case to motivate the proposed approach. We also propose a specification language called Cyberlog to monitor the dynamic behavior of the system. On the other hand, the evaluation experiment in Chapter 5 is somewhat questionable, since the proposed method is implemented in the RTAPHM system, but the analysis is based only on the processing delay and the amount of facts. Furthermore, in Chapter 6, related studies are abruptly introduced, which may confuse the readers.



----------------------- REVIEW 2 ---------------------
SUBMISSION: 5585
TITLE: Monitoring Auditable Claims in the Cloud
AUTHORS: Lev Sorokin and Ulrich Schöpp

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
Paper summary:
The paper presents a system for monitoring claims in a distributed system.

Strengths:
+ The approach is an interesting software architecture for exchanging/testing claims between different systems

Weaknesses:
- The solution contains only little original research contribution

Detailed comments:
* The paper states that the attestations are cryptographically signed, but no details are given.
* The solution seems to be mainly aligned with the project use case
* Prior work is claimed to be not performant enough, but no comparison with the one solution is given
* The terms "security" and "safety" are used inconsistently
* The comparison with certificate transparency is not convincing



----------------------- REVIEW 3 ---------------------
SUBMISSION: 5585
TITLE: Monitoring Auditable Claims in the Cloud
AUTHORS: Lev Sorokin and Ulrich Schöpp

----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
The paper aims at monitoring safety and data-related properties in a mission-critical environment deployed on clouds. The paper claims to be not scoped by specific implementations, as those implementations may vary from each other as well as change with frequent updates. It adds a verification layer to the cloud system to enable monitoring its operations (based on events).

Thus, the paper seems to target an important domain with a critical application into consideration. However, the writing and organization of the paper can further be improved - now several cases the flow is not perfect. The list of contributions in the intro do not directly match with he motivation and problem statement - how “introducing a new datalog-based language” was needed is not clear from the paper. The overall description of the paper is going back and forth form high-level (mission critical systems in cloud) to low-level (UAV) without clear separation between them - so readability is compromised time to time. Challenges to generalize Certification Transparency project in this context might be very valuable, as that seems to be the main contribution of the paper. Section 2 is better to cal motivating example - as it seems to be the purpose. The current title (use case) is bit confusing. Preferably avoid using past tense in the intro and earlier section, unless es
sential.


----------------------------------------

Summary
- To much coupled with the RTAPHM use case
- Generalizability of CT not clear
- Not clear why cyberlog is introduced
- "Contributions do not match with problem statement"
- "The current title (use case) is bit confusing."
- grammar
- "in Chapter 6, related studies are abruptly introduced, which may confuse the readers"
- "The paper states that the attestations are cryptographically signed, but no details are given."

==> sketch.tex <==
AFML ähnlicher use cases als besserer Use case, ohne revision?

-> Supply chain security (trillian use cases: ChecksumDB, FirmwareDB)


SolarWinds and others led to the compromise of numerous other organizations. A malicious update, allowed the remote access of a trojan to infect all the customers systems and networks. Software supply chain attacks like this pose a serious threat to governments, companies, non-profits, and individuals. Monitoring supply chains is a complex endeavor as it requires use of case-specific implementation of monitoring code to provide security guarantees. 

We propose a framework for flexible monitoring of auditable claims to provide supply chain security. Our approach is based on the execution of distributed Datalog programs in connection with the tamper-proof storage Trillian. Our approach can be seen as a generalization of the widely applied Certificate Transparency project where publicly issued HTTPS certificates are monitored to identify maliciously issued certificates. We demonstrate our framework by applying it to two scenarios that enable firmware transparency.


########################
What are the contributions:
 - Specification in the Datalog the monitoring workflows
 - Each monitoring request root hash from Trillian, makes inclusion proofs
 - What about the REST interface?

From Reviews:
 - Compare to Certificate Transparency
 - Explain Cryptographical Signature
 - Safety <-> Security
 
